Challenges and Opportunities for RISC-V Architectures towards Genomics-based Workloads

The use of large-scale supercomputing architectures is a hard requirement for scientific computing Big-Data applications. An example is genomics analytics, where millions of data transformations and tests per patient need to be done to find relevant clinical indicators. Therefore, to ensure open and broad access to high-performance technologies, governments, and academia are pushing toward the introduction of novel computing architectures in large-scale scientific environments. This is the case of RISC-V, an open-source and royalty-free instruction-set architecture. To evaluate such technologies, here we present the Variant-Interaction Analytics use case benchmarking suite and datasets. Through this use case, we search for possible genetic interactions using computational and statistical methods, providing a representative case for heavy ETL (Extract, Transform, Load) data processing. Current implementations are implemented in x86-based supercomputers (e.g. MareNostrum-IV at the Barcelona Supercomputing Center (BSC)), and future steps propose RISC-V as part of the next MareNostrum generations. Here we describe the Variant Interaction Use Case, highlighting the characteristics leveraging high-performance computing, indicating the caveats and challenges towards the next RISC-V developments and designs to come from a first comparison between x86 and RISC-V architectures on real Variant Interaction executions over real hardware implementations.

==> background.tex <==
\section{Variant Interaction Analytics (VIA) Workload}
\label{sec:background}

%- Definition of MEEP

%- Definition of WP5 + tasques nostres

%- Definition of Epistasia APP
\subsection{The method}
The method that we are applying for detecting variant-variant interaction is the MDR. With the aim of improving the power to detect variant-variant combinations, MDR is a statistical method that, based on contingency tables, reduces the dimension of the problem. More specifically, it converts the counts obtained for the cases and controls into a simple binary variable by classifying all the possible allelic combinations for each pair in high-risk/low-risk, therefore, reducing the analysis to only one dimension. It follows a naive Bayes approach, building a probabilistic classifier from every variant-variant interaction and summarizing the best combinations for prediction.

As illustrated in fig.\ref{fig:mdr_steps}, the method can be divided into 5 different steps: 
\begin{itemize}
    \item The first step consists of dividing the data into a training set and a testing set for a k-fold cross-validation. This step is done to avoid potential over-fitting and, therefore, to find pairs of variant-variant combinations that can have an effect on any dataset, not just the one being evaluated. 
\end{itemize}

Steps (2-4) are going to be performed k-times, one for each distribution of the training and the testing within the k-fold cross-validation. 
\begin{itemize}
    \item In the second step we will build a contingency table for each of the evaluated variant-variant pairs. In the problem of variant-variant interaction, we are working with a 2 factors table (variant-variant), each one with 3 classes corresponding to the variant genotypes (AA, Aa, aa), ending with a 9 cells table called multifactor classes. Then, each multifactor class is going to be filled with the number of cases and controls found in the training dataset that belongs to each class, thus, building the 2-dimensional table. 
    \item In step three the tables are going to be transformed into a 1-dimension space using the original cases and control distribution of the dataset as a threshold, T. The cells where the ratio of cases to controls is bigger than the threshold is going to be classified as ‘high risk’ and as ‘low risk’ if the ratio is lower than the threshold.
    \item Now that the dimension of the table has been reduced, in step four each of the variant-variant tables is used to classify the testing set of the data and sort all the variant-variant tables using the prediction error, getting the best variant-variant combination for this cross-validation set.
\end{itemize}

\begin{figure*}[ht]
\captionsetup{font=footnotesize}
  \includegraphics[width=\textwidth]{FIG/mdr_steps.png}
  \caption{Multifactor Dimensionality Reduction algorithm steps. Step 1 is the cross-validation division. Step 2 is the building of contingency tables. In step 3, the dimension of the contingency tables is reduced to 1. In step 4, each multifactor is tested. Steps 2-4 are repeated for each cross-validation set and in Step 5, the top pairs are selected.}
  \vspace{-2em}
  \label{fig:mdr_steps}
\end{figure*}

Then, step two, three, and four are repeated for each of the possible cross-validation sets from step one,   
\begin{itemize}
    \item In step five the best and most consistent variant-variant combinations are selected, which means picking the ones that appear in the most cross-validation sets as a top pair. Particularly, in a 5-fold cross-validation, being in the top has been defined as being in the top 20\% of pairs with the smaller prediction error.
\end{itemize}

\subsection{The framework}

The method has been developed leveraging Apache Spark framework for parallel computation \cite{spark}. Apache Spark is an open-source distributed processing system for high-volume workloads. Thanks to its in-memory caching and a system of optimized queries, it can be used against data of any size. It has a master-slave architecture, combining a single master with multiple slaves.






==> benchmarking_backup.tex <==
\section{Benchmarking Methods}
\label{sec:methodology} 

\subsection{Variant-Interaction Analytics Workload Pipeline}
The first step in the Variant-Interaction Analytics (VIA) Workload is loading the labels of the data. From them, we extract the number of patients that we have and generate 5 different train and test sets to perform a 5-fold cross-validation (CV). Then, we get the ratio, T, of cases and controls, which will be then used for performing the dimensionality reduction. Once we have this information, the VIA workload begins to load the first file that needs to be processed and executes the MDR algorithm against a second file, processing every possible pairwise combination between both files. From this process, the workload stores five different prediction errors for each SNP combination, one for each CV fold. This is the output of the Variant-Interaction Analytics workload.

The process of computing a pair of variants does not imply a lot of memory or computational power. However, the high volume of pairs of variant combinations that we need to process demands the use of High-Performing Computing (HPC) technologies to make it feasible (see the description of the data at the end of this section)., Since processing a pairwise combination of variants is computationally independent of the following combinations, we can use parallel computation frameworks such as Apache Spark. Using an RDD to store the combinations allows us to apply a map function and assign the available workers to different partitions of the RDD. Due to this independence of the combinations, we can also scale it down to test it in different architectures and extrapolate the results to real-case scenarios.

\subsection{Dataset}

The dataset used for the benchmarking experiments is a synthetic dataset based on the Northwestern NuGENE project cohort \cite{nugene}. Maintaining the structure and the number of patients we have recreated a single chromosome using randomized values for the new synthetic patients. The data is stored in compressed CSV format, following the structure in table \ref{tab:data}. Each line corresponds to a variant and is composed of 5 columns with the identification and information about the characteristics of the variant, followed by the value of the variant for each of the patients of the dataset. 

\begin{table*}[]
\hspace{0em}
\centering
\captionsetup{font=footnotesize}
\begin{tabular}{ccccccccccccccccc}
\hline
chromosome & variant pos.   & Ref hom & Alt hom & AA & Aa & aa & AA & Aa & aa & ... & AA & Aa & aa \\
\hline

22         & 16231367   & A       & G       & 1       & 0       & 0       & 1       & 0       & 0       &     & 0       & 1       & 0  \\
22         & 17052123   & G       & A       & 0       & 1       & 0       & 0       & 0       & 1       &     & 0       & 0       & 1  \\
22         & 17055458   & G       & A       & 0       & 1       & 0       & 1       & 0       & 0       &     & 0       & 1       & 0  \\
22         & 17055984   & C       & T       & 0       & 1       & 0       & 1       & 0       & 0       &     & 1       & 0       & 0  \\
22         & 17056038   & G       & A       & 1       & 0       & 0       & 0       & 0       & 1       &     & 1       & 0       & 0 \\
\hline \\
\end{tabular}
\captionof{table}{first five rows of synthetic chromosome 22. The first column is the number of the chromosome, the second column is the position of the variant. The third column is the homozygous reference allele, and the fourth column is the homozygous alternative allele. The following columns are structured in blocks of three, one block per patient for a total of 1,128 patients. The first column of the block is the value for case AA of both alleles being the reference one. The second column is the value for case Aa, where one allele is the reference and the other the alternative, and the last column is for the case where both alleles are the alternative. The total number of columns is  3,389.} \label{tab:title} 
\vspace{-2em}
\label{tab:data}
\end{table*}

The labels of the data are saved in a different file, including the patient ID and a binary marker that indicates if the patient is a case or a control. A cohort such as NuGENE is composed of 11,297,253 SNPs, forming a dataset of 11,297,253 rows x 3,389 columns. In a variant interaction analysis, we are studying the association between each pairwise interaction with the disease, which means that in the most simple case, we are going to process every possible pair. This means that the number of combinations ascends approximately to (11,297,253 x 11,297,252)/2 = 63,813,957,024,378. The synthetic dataset created for the benchmark is a reduced version, generating 10 files of 50 SNPs with all the patients. We have not decreased the number of patients because maintaining the same structure allows us to easily extrapolate the computation time just by multiplying the number of files that need to be processed.




==> conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}

In this paper, we have introduced Variant-Interaction Analytics Workload (VIA), a relevant genomics-HPC workload. The first challenge explored is how to characterize its performance on RISC-V development platforms and fairly compare it to more mature and production-ready x86 platforms. We have explained that the dataset must be reduced in a way that is still representative of real-world environments, despite being considerably smaller. This allows us to run the workload on RISC-V platforms within a reasonable time and to be still able to compare the results to real-world scenarios.
Secondly, we have characterized the main existing differences between RISC-V platforms and x86 and adapted the workload appropriately to produce x86 results that could be fairly compared to RISC-V results. This has allowed us to see the challenges that RISC-V still faces to become a realistic alternative to x86 in HPC environments.
As a result, we have seen that one of the main challenges is the lack of a full one-to-one match on instructions available on x86 compared to RISC-V, with special mention of the lack of vectorial extension support on our evaluated RISC-V platform. Additionally, we have seen that moving data across multiple nodes is a challenge RISC-V still has to face, as its data transfer speed is lower than the available on x86 platforms.
Finally, we have produced an open-data repository \cite{openrepo_rv_genomics} that allows us to access all the experimental data obtained so far and to reproduce the results on other RISC-V and x86 platforms. 
